Distributed State Estimation for Linear Time-Varying Systems with Sensor Network Delays

Distributed sensor networks often include a multitude of sensors, each measuring parts of a process state space or observing the operations of a system. Communication of measurements between the sensor nodes and estimator(s) cannot realistically be considered delay-free due to communication errors and transmission latency in the channels. We propose a novel stability-based method that mitigates the influence of sensor network delays in distributed state estimation for linear time-varying systems. Our proposed algorithm efficiently selects a subset of sensors from the entire sensor nodes in the network based on the desired stability margins of the distributed Kalman filter estimates, after which, the state estimates are computed only using the measurements of the selected sensors. We provide comparisons between the estimation performance of our proposed algorithm and a greedy algorithm that exhaustively selects an optimal subset of nodes. We then apply our method to a simulative scenario for estimating the states of a linear time-varying system using a sensor network including 2000 sensor nodes. Simulation results demonstrate the performance efficiency of our algorithm and show that it closely follows the achieved performance by the optimal greedy search algorithm.

==> newintro.tex <==
The general concept of distributed estimation and control \cite{Olfati1} is that it is possible to produce estimates of the states of any dynamical system through communication between sensor nodes. These estimation techniques are shown to be far more reliable and robust compared to their conventional counterparts. In addition, it has also been proven to be scalable with the size of the network \cite{talebi}, making it effective even with dense sensor networks. These estimation techniques \cite{hao} using sensor networks are broadly classified into two categories: centralized and decentralized. In the former, there exists communication between each sensor node and a "fusion" centre, that computes an estimate of the state dynamics. While this method requires fewer computations, it may not be dependable, as a single node failure could bring the entire system down \cite{speranzon}. In addition, centralized algorithms have scalability issues \cite{hao}. To tackle these problems, decentralized or distributed Kalman filtering algorithms in \cite{talebi,Olfati1,MesbahiEgerstedt+2010} have been proposed. The main idea behind the Distributed Kalman Filter (DKF) is that sensor nodes mutually exchange information with their neighbours and produce estimates of the state as well as the covariance matrices. Such an information fusion technique makes the estimation process more reliable, in the sense that a few node failures only lead to local inaccuracies. DKF architectures make the estimation process more dependable and robust by the elimination of a single fusion centre. However, these are also affected with the burden of communication overload in dense sensor networks.
